QuadConv: Quadrature-Based Convolutions with Applications to Non-Uniform PDE Data Compression

We present a new convolution layer for deep learning architectures which we call QuadConv -- an approximation to continuous convolution via quadrature. Our operator is developed explicitly for use on non-uniform, mesh-based data, and accomplishes this by learning a continuous kernel that can be sampled at arbitrary locations. Moreover, the construction of our operator admits an efficient implementation which we detail and construct. As an experimental validation of our operator, we consider the task of compressing partial differential equation (PDE) simulation data from fixed meshes. We show that QuadConv can match the performance of standard discrete convolutions on uniform grid data by comparing a QuadConv autoencoder (QCAE) to a standard convolutional autoencoder (CAE). Further, we show that the QCAE can maintain this accuracy even on non-uniform data. In both cases, QuadConv also outperforms alternative unstructured convolution methods such as graph convolution.

==> review.tex <==
Reviewer #1: The paper proposes a novel convolution layer suitable for non-uniform, mesh-based data by learning a continuous kernel and quadrature rule. The authors provide numerical examples based on PDE simulation data that demonstrate the effectiveness of the proposed method on both uniform and non-uniform mesh data.

The idea is interesting. I have the following comments:


1.In equation (6) on page 7, it would be helpful if the authors could provide guidance on how to choose the parameter \alpha in practice, especially for new problems. Additionally, it would be useful to know what specific values of alpha were used in the examples presented later in the paper.

2. On page 8, the authors mention that it is possible to construct node-based quadrature weights from individual element quadrature evaluations for data from FEM-based simulations, but this procedure can be complicated and computationally intensive. It would be beneficial if the authors could elaborate on why this procedure is complex since this procedure is a standard task in FEM simulations.

3. It is unclear from the paper whether this approach can handle data from adaptive meshes. It would be helpful if the authors could provide more insights on this matter and discuss any potential challenges that may arise when dealing with adaptive meshes.



Reviewer #2: Summary
This paper presents the incorporation of quadrature approximation into the graph convolution of field signals on a non-uniform grid. The proposed method involves learning quadrature coefficients and a continuous kernel, which are then applied to flow data compression. The results demonstrate competitive performance compared to traditional convolutional neural networks. The paper has a clear structure and is easy to read. However, the reviewer has several major concerns that need to be addressed before it can be considered for publication.
Comments

Major comments:
1. The reviewer raises a significant concern regarding the thoroughness of the literature review presented in the paper. In particular, in section 1.2 on page 5, the author suggests that spatial graphs with non-trivial down-sampling steps are unsuitable for spatially embedding data. However, the reviewer argues that the term "non-trivial" does not automatically imply unsuitability, as previous graph convolutional operators based on adjacency structures can be readily applied once a down-sample algorithm is established. The authors are not aware of that there are intensive research on numerous down-sampling algorithms, often referred to as multi-scale GNN or Graph U-net approaches. Some notable examples include MeshCNN by Hanocka et al. (https://arxiv.org/abs/1809.05910) and Coma by Ranjan et al. (https://arxiv.org/pdf/1807.10267.pdf). Moreover, researchers have also formulated data on point clouds and utilized message passing on k-nearest-neighbor graphs, as exemplified in, e.g., (https://arxiv.org/pdf/2212.05023.pdf). One advantage of this alternative is its potential to significantly reduce computational costs by focusing solely on local neighborhoods. In light of these observations, the reviewer suggests that the authors should overhaul the literature review, better justify why the proposed method is valuable on the top of the existing literature, and compares the proposed method with the aforementioned previous models in the results section comprehensively (data efficiency, accuracy, generalizability, memory footprint etc).
2. There is concern regarding the literature review's coverage of continuous convolution (as mentioned in the 3rd row of Page 6), as the authors primarily reference several very recent (2022) publications (references 14, 15, and 16), which is a little bit misleading may give the audience a wrong impression that continuous convolution is somewhat a new concept. In fact, continuous convolution operators have been extensively studied in both the computer science, computer vision, and recently computational physics communities. In the computer science community, spatial continuous kernels on GNNs were introduced as early as 2017 (https://arxiv.org/pdf/1704.02901.pdf). One well-known example is SplineCNN by Fey et al. (https://arxiv.org/pdf/1711.08920.pdf), which has already been incorporated into the official library in PyTorch Geometric package for years. In the physics modeling community, Li et al. also revisit the same concept (i.e., continuous kernels for graph convolution) for learning operators (https://arxiv.org/pdf/2003.03485.pdf). Given these important contributions, it is crucial for the author to thoroughly revise the literature review and address this concern. The revised section should acknowledge the existence of these previous works and provide a comprehensive overview of the research on continuous convolution. It is essential to highlight the early works in the field, such as the 2017 publication on spatial continuous kernels and the subsequent advancements.
3. A global graph convolution operator is used but Figure 4b indicated a local quadrature convolution. The authors may want to modify Figure 4 by changing the reception field of the red node to be the entire mesh, thus representing a global graph convolution.
4. The reviewer acknowledges the rationale behind the idea of quadrature-based convolution, which provides a better approximation of convoluted results in each output channel. However, they raise a valid concern regarding the feasibility of incorporating quadrature-based convolution into neural networks (NNs). While a QuadConv layer may improve the approximation of a continuous convoluted signal in each output channel, it does not necessarily guarantee better overall fitting results for the entire NN. The reviewer questions the practicality of this idea, particularly when compressing transient CFD data on a single mesh, which is often the case in data compression. It seems a regular CNN, which learns the specific discrete representation of the data, can perform well. The learning process of a regular CNN is limited to the specific discrete point distribution (in multi-scale) and does not require consideration of continuous field approximations. This is likely the reason why the proposed method fails to outperform a regular CNN, as indicated in Table 2. Consequently, the reviewer suggests the authors to consider scenarios involving multiple discrete representations. This could include cases where different parts of the CFD data are valued on different meshes or situations where the trained model is applied to a re-meshed domain. The reviewer recommends conducting test cases to demonstrate this comparison.
5. The author underscores a significant advantage of the proposed Quadrature Convolution (QuadConv): the freedom to select output points irrespective of the input points. Although two pages were devoted to promoting QuadConv, it's claimed that this method learns quadrature weights which are more efficient in restoring the field post-convolution. The argument suggests that, if finite points are predetermined, it eliminates the necessity to learn weights as they can be deterministically calculated. In Example 3.1, identical input and output points are presented, and the max pooling function easily manages the pooling layer. However, in Example 3.2, only the first and last QuadConv layers have differing input and output points, serving merely as an interpolation between non-uniform and uniform grids. This implementation of QuadConv seems trivial given that one could simply apply cubic interpolation to transform a non-uniform grid to a uniform one and subsequently use a Convolutional Neural Network (CNN) for the task. Example 3.3 use QuadConv for down-sampling, yet the output point remains a subset of the input point, eschewing the opportunity to independently sample new output points. The reviewer requests clarification on why QuadConv wasn't utilized as an up or down sampling layer until Example 3.3, and why the choice was made to employ subsampling over independent sampling. New experiments should be conducted and more evidences are needed to support the author's claim.
6. The reviewer believes that readers would be keen to understand how state-of-the-art graph learning algorithms fare in the realm of data compression. Consequently, in addition to the Convolutional Neural Network (CNN), the reviewer encourages the author to incorporate the following baselines:
a. Proper Orthogonal Decomposition (POD)
b. A standard Graph Convolutional Network (GCN) or variants like Graph Attention Networks (GAT), Graph Isomorphism Network (GIN), or MeshGraphNet, supplemented by a graph pooling algorithm
c. Graph K-Nets (GKN) from Li et al. (https://arxiv.org/pdf/2003.03485.pdf)
These should be tested on all use cases. The author needs to substantiate the superiority of their method over previous works to highlight their contribution. A comparison involving re-meshed inference should also be included.
7. Despite the introduction of a symbolic calculation of operation cost in Table 1, the reviewer is interested in a comparison of the training and inference speeds between the proposed method and the established baselines across all test cases. Given that this paper focuses on non-uniform PDE data compression, the practical use cases will generally involve more complex scenarios such as 3-D unstructured meshes with more complicated physics. For instance, the Reynolds number in case 3.3 is merely 100, and the flow is very periodic and less interesting. The reviewer recommends that the author evaluates the proposed model in more non-periodic regime. Plenty of reduced-order models have been showed to deal with 2D/3D turbulence, which is a context where the proposed data compression method is expected to apply.
8. The author should provide a detailed report on the training and inference cost comparison for all test cases and all different models. This report should include significant amount of details such as the number of trainable parameters, training time, RAM used, inference time, and so on.


Minor comments:
1. The reviewer recommends that the author create distinct figures to visually represent any modifications made to the original model depicted in Figure 6. As it stands, various models are textually described within three separate cases, which may not provide a clear, intuitive understanding.
2. For Figures 7, 10, and 12, the reviewer suggests increasing the size of the text to enhance readability.
